Approximation Algorithms for Multiprocessor Scheduling under Uncertainty

Motivated by applications in grid computing and project management, we study multiprocessor scheduling in scenarios where there is uncertainty in the successful execution of jobs when assigned to processors. We consider the problem of multiprocessor scheduling under uncertainty, in which we are given n unit-time jobs and m machines, a directed acyclic graph C giving the dependencies among the jobs, and for every job j and machine i, the probability p_{ij} of the successful completion of job j when scheduled on machine i in any given particular step. The goal of the problem is to find a schedule that minimizes the expected makespan, that is, the expected completion time of all the jobs. The problem of multiprocessor scheduling under uncertainty was introduced by Malewicz and was shown to be NP-hard even when all the jobs are independent. In this paper, we present polynomial-time approximation algorithms for the problem, for special cases of the dag C. We obtain an O(log(n))-approximation for the case of independent jobs, an O(log(m)log(n)log(n+m)/loglog(n+m))-approximation when C is a collection of disjoint chains, an O(log(m)log^2(n))-approximation when C is a collection of directed out- or in-trees, and an O(log(m)log^2(n)log(n+m)/loglog(n+m))-approximation when C is a directed forest.

==> sch-tree.tex <==
\junk{
With the chain decomposition result of Kumar et al.~\cite{KumarEtAl05},
we can also extend our results for the chain case to the more general
case where the precedence constraints are tree-like structures, i.e.,
directed forest. We simply decompose the jobs into at most $\gamma=
O(\log n)$ blocks, and within each block, apply our algorithm for the
chain case (Theorem~\ref{thm:chain}). Since the optimal expected
makespan on any subgraph (subset of jobs) is a lower bound for that of
the whole graph (whole set of jobs), this approach gives up another
factor of $\log n$. We have thus obtained

\begin{theorem} \label{thm:forest} For Problem {\suu}, if the
  dependency graph $C$ is a directed forest, an {\oblivs} can be
  computed within polynomial time, whose expected makespan is within a
  factor of $O(\log m\log^2 n\frac{\log (n+m)}{\log\log (n+m)})$ of
  the optimal.
\end{theorem}
}

%%\subsection{tree constraints}

Recall that our approach to the {\suu} problem with constraints is as
follows: We solve a relaxted LP program to obtain an integral
solution, whose load (and length) is bounded by the optimum; The
integral solution gives us a pseudo-schedule, which can be converted
to a feasible schedule based on random delay argument; Finally we
replicate our schedule in order to finish all jobs with high
probabilities.

\junk{
tree case
complexity
proof reading
adaptive proof

close to end of section 1.1, ``Wel'' -> ``We''
proof of theorem 3.3, ``By Theorem''?
Proof for SUU-I-OBL in appendix: now we have n/16, not n/4

one way of fix:

replace 1/4 by 1/16
replace 1/24 by 1/96
replace 1/23 by 1/95
replace 16log n by 66log n (notice also algorithm 2)
replace 90log n by 362log n 
(1-1/96e)^181 < 1/2


}

For the scheduling problem on unrelated machines when the precedence
constraits form a collection of {\em out trees} (rooted trees with
edges directed away from the root) or {\em in trees} (defined
analogously), Kumar et al.~\cite{KumarEtAl05} obtain an improved
approximation algorithm as follows. Decompose the out/in trees into
$O(\log n)$ blocks; Randomly delay each chain by an amount of steps
chosen uniformly from $[0, O(\Pi_{max}/\log n)]$ (This step can be
derandomized in polynomial time); Prove that with high probability, at
most $O(\log n)$ jobs can be scheduled on any machine simultaneously.
With similar ideas and arguments, we also obtain an improved
approximation bound for the tree case. We defer the details to the
full version.

\begin{theorem} \label{thm:tree} For Problem {\suu}, if the dependency
  graph $C$ is a collection of out/in trees, an {\oblivs} can be
  computed within polynomial time, whose expected makespan is within a
  factor of $O(\log m\log^2 n)$ of the optimal.
\end{theorem}

